Leveraging Class Hierarchies with Metric-Guided Prototype Learning

In many classification tasks, the set of target classes can be organized into a hierarchy. This structure induces a semantic distance between classes, and can be summarised under the form of a cost matrix, which defines a finite metric on the class set. In this paper, we propose to model the hierarchical class structure by integrating this metric in the supervision of a prototypical network. Our method relies on jointly learning a feature-extracting network and a set of class prototypes whose relative arrangement in the embedding space follows an hierarchical metric. We show that this approach allows for a consistent improvement of the error rate weighted by the cost matrix when compared to traditional methods and other prototype-based strategies. Furthermore, when the induced metric contains insight on the data structure, our method improves the overall precision as well. Experiments on four different public datasets - from agricultural time series classification to depth image semantic segmentation - validate our approach.

==> 3_method.tex <==
%In this section, we present our approach to incorporate the error metric into a classification model.
We consider a generic dataset $\cN$ of $N$ elements $x \in \cX^\cN$ with ground truth classes $z \in \cK^\cN$.
We assume that the cost matrix $D\in \bR_+^{K\times K}$ is symmetric, \ie misclassifying class $k$ for class $l$ or the contrary has the same cost.% as misclassifying $l$ for $k$. 
We also assume that $D$ respects the triangle inequality and thus that $(\cK, D)$ defines a finite metric space. Cost matrices which do not respect these two conditions are out of the scope of this paper.
%\SOUT{respects the triangle inequality, \ie that $(\cK, D)$ is a finite metric space.}
%
We denote by $\Omega$ the \emph{embedding space} which, when equipped with the distance function $d:\Omega\times\Omega \mapsto \mathbb{R}_+$, forms a metric space as well.
%
%...................................................
\subsection{Prototypical Networks}
%...................................................
A prototypical network is characterized by an embedding function $f:\cX\mapsto\Omega$, typically a neural network, and a set $\pi\in\Omega^\cK$ of $K$ prototypes.
$\pi$ must be chosen such that any sample $n$ of a given class $k$ has a representation $f(x_n)$ which is \emph{close} to $\pi_k$ and \emph{far} from other prototypes.

Following the methodology of \citet{snell2017prototypical}, a prototypical network $(f,\pi)$ associates to an observation $x_n$ the following posterior distribution over its class $z_n$:
\begin{align}
\label{eq:proba}
   p(z_n=k| x_n)   &= 
   \frac{\exp{\left(-d\left(f(x_n),\pi_{k}\right)\right)}}
   {\sum_{l \in \mathcal{K}}\exp{\left(-d\left(f(x_n), \pi_{l}\right)\right)}}~, \forall k \in \cK~.
\end{align}
We can then define an associated loss with the normalized negative log-likelihood of the true classes:
\begin{align}
    \Ldata(f,\pi)
    %&=
    %\frac{-1}{N} \log\left( p\left(\{y_n\}_{i \in \cN}| \{x_n\}_{n \in \cN}\right)\right)\\
    &=
    \frac1{N} \sum_{n \in \cN}
    \left( d(f(x_n), \pi_{z_n})
    +
    \log\left(\sum_{l\in \cK} \exp{(-d(f(x_n), \pi_{l}))}\right)\right)~.
    \label{eq:ldata_long}
\end{align}
This loss is such that the representation $f(x_n)$ is attracted towards the prototype of the class $z_n$, while it is repelled by the other prototypes.
Conversely, prototype $\pi_k$ is drawn towards the representations $f(x_n)$ of samples $n$ of class $k$ and away from the  representations of other classes.
%In previous work of the literature, the prototypes are directly defined as centroids of the embeddings of the elements of their classes, and updated at each episode \cite{snell2017prototypical} or iteration \cite{guerriero2018deepNCM}.\footnote{which corresponds to an alternate optimization scheme between the embedding function and the prototypes.} In the work of Mettes \etal \cite{mettes2019hyperspherical}, the prototypes are defined prior to learning the embedding function.

In contrast to previous work on prototypical networks which learn  prototypes separately or define them as centroids of representations, we propose to learn the embedding function $f$ and the prototypes $\pi$ \emph{simultaneously}. 
This allows us to learn prototypes which take into account both the distribution of the data and the relationships between classes, as described in the next section. Furthermore, this removes the need for keeping track of the average representation of each class.
%......................................................
\subsection{Metric-Guided Penalization}
%......................................................
\label{sec:disto}
%Next, we use these learnt prototypes to structure the embedding space according to the finite metric over classes $\delta$. Specifically, we want to assess whether placing prototypes in the embedding space consistently with the hierarchical distance between the corresponding classes helps in reducing the empirical hierarchical cost of prediction. 
%
%\paragraph{Distortion loss}
%
%We propose to do so by realizing the finite metric defined by $D$ over $\cK$ in the embedding space $\Omega$. This is achieved by minimizing the distortion between the inter-class distances in $\cK$ and the corresponding inter-prototype distances in $\Omega$. This task is also known as the \textit{ realization} of a graph into a metric space. The distortion of a graph-realization is commonly defined as per Eq. \ref{eq:disto}. It measures the average scaled absolute difference between the length of a graph edge and the norm of its realization in the embedding space. We adapt the formula of the distortion into a loss term $\Ldisto$ (Eq. \ref{eq:ldisto}) by taking the squared differences instead of absolute values. 
%
%
%\begin{align}
%    \Delta(\pi, {D}) &= \frac{1}{\vert K \vert^{2}-\vert K \vert} \sum\limits_{k,l \in \cK^2, k\neq %l} \frac{\left\vert d(\pi_{k},\pi_{l}) - D_{k,l}\right\vert}{D_{k,l}}   \label{eq:disto}\\
%    \Ldisto(\pi, {D}) &= \frac{1}{\vert K \vert^{2}-\vert K \vert} \sum\limits_{k,l \in \cK^2, k\neq %l} \left(\frac{ d(\pi_{k},\pi_{l}) - D_{k,l}}{D_{k,l}}\right)^2 \label{eq:ldisto}
%\end{align}
%
\SCALE{
We propose to incorporate the cost matrix $D$ into a regularization term in order to encourage the prototypes
%We propose to incorporate the cost matrix $D$ into a regularization term.  \VIVIEN{It encourages} the prototypes  $\pi$ % \VIVIEN{, and indirectly the sample representations,} 
to organize in the embedding space $\Omega$ in a manner that is consistent with the finite metric defined by $D$. Since sample representations are attracted to their respective prototypes in \eqref{eq:ldata_long}, this regularization also affects the embedding network.
%
\paragraph{Distortion}
As described in \citet{de2018representation}, the distortion of a mapping $k \mapsto \pi_k$ 
between a finite metric space $(\cK, D)$ and a continuous metric space $(\Omega,d)$ can be defined as:
\begin{align}
\label{eq:disto}
\text{disto}(\pi,D) = \frac1{K(K-1)}
\sum_{k,l \in \cK^2,\,k\neq l} \frac{\left\vert d(\pi_{k},\pi_{l}) - D[k,l]\right\vert}{D[k,l]}~.
\end{align}
If the mapping defined by $\pi$ has low distortion, the distances $d$ between prototypes are close to the cost between their respective classes as defined by $D$.
Consequently, misclassifying a sample $x_n$ of class $k$ with a high-cost class would require $f(x_n)$ to be further away from $\pi_k$ than for another class with a lower cost. 
%\VIVIEN{Thus defined, distortion measures both how well the distance ratios are preserved by the mapping and }

%In practice, the distortion should be independent of the scale of either metrics and measure how well the distance ratios are preserved by the mapping, see our scale-independent distortion detailed in the Appendix.
%
\paragraph{Distortion-Based Penalization:} 
%\LOIC{In practice, the distortion should be independent of the scale of either metrics and measure how well the distance ratio are preserved by the mapping, see our scale-independent distortion detailed in the Appendix.
%the measure of the distortion should be independent of the scale of either metrics, as measured by the our scale-free distortion detailed in the Appendix.
%However,}
\equaref{eq:disto} leads us to a straightforward way of incorporating the error qualification in the prototypes' representations with the following smooth regularizer:
\begin{align}
\label{eq:loss:disto}
    \Ldisto(\pi) &=
    \frac{1}{K(K-1)}
\sum_{k,l \in \cK^2,\,k\neq l} \left(\frac{ d(\pi_{k},\pi_{l}) - D[k,l]}{D[k,l]}\right)^2~.
\end{align}
However, this loss imposes specific distances between prototypes, conflicting with the second term of $\Ldata$ which encourages distances between embeddings and unrelated prototypes to be as large as possible. As a consequence, these two losses can not be simultaneously zero, even asymptotically. 

%, a low distortion is not necessary to decrease the likelihood of confusing \emph{distant} classes.
\paragraph{Rank-Based Penalization:}
Following the ideas of  \citet{mettes2019hyperspherical}, we also define a RankNet-inspired loss \citep{ranknet} which encourages the distances between prototypes to follow \emph{the same order} as the costs between their respective classes, without imposing a specific scaling: 
\begin{align}\label{eq:loss:rank}
    \Lrank(\pi) &= - \frac{1}{\vert\cT\vert }
\sum_{k,l,m \in \cT} %\left( 
\bar{\bf R}_{k,l,m} \cdot \text{log}(R_{k,l,m}) + (1 - \bar{\bf R}_{k,l,m}) \cdot \text{log}(1- R_{k,l,m}) %\right)
~,% \\
    %& \cT \subset \{(i,j,k) \in \cK^3 | i \neq j, j \neq k , k\neq i \} \nonumber \\
    %\bar{R}_{i,j,k} & = [\![ D_{i,j} > D_{i,k} ]\!]  \label{eq:rbar}\\
    %R_{i,j,k} &= \text{sigmoid}(d(\pi_i,\pi_j) - d(\pi_i,\pi_k))  
\end{align}
with $\cT=\{(k,l,m) \in  \cK^3\mid k\neq l, l\neq m, k\neq m\}$ the set of ordered triplet of $\cK$,  $\bar{\bf R}_{k,l,m}$ the hard ranking of the costs between $D_{k,l}$ and $D_{k,m}$, equal to $1$ if $D_{k,l} > D_{k,m} $ and $0$ otherwise, and $R_{k,l,m} = \text{sigmoid}(d(\pi_k,\pi_l) - d(\pi_k,\pi_m))$ the soft ranking between $d(\pi_k,\pi_l)$ and $d(\pi_k,\pi_m)$.
For efficiency reasons, we sample at each iteration only a $S$-sized subset of $\cT$.
\VIVIEN{For a measure of how well the distance ratios are preserved by the mapping, see our scale-independent distortion detailed in the Appendix}

%\paragraph{Hidden prototypes:} In cases where the cost matrix $D$ is derived from a tree-shaped class hierarchy, it is possible to also learn prototypes for the internal nodes of this tree, corresponding to super-classes of leaf-level labels. These prototypes do not appear in $\Ldata$, but can be used in the prototype penalization to instill more structure into the embedding space.

%The interest of the rank-based approach in $\Lproto$ is to influence the pairwise distances between prototypes only on a relative scale and thus avoid a potential conflict with $\Ldata$. 

%We use the prototypes to incorporate information about class relationships during the joint learning of the embedding function and the prototypes. To this end, we use a regularization term $\Lproto$ which aims at organizing the prototypes in the embedding space, consistently with the distances between classes  given by $D$. Following \cite{mettes2019hyperspherical} we propose to supervise the prototypes with a RankNet \cite{ranknet} inspired ranking loss. This second loss term $\Lproto$ encourages the pairwise distances in triplets of prototypes to rank in the same order as the corresponding hierarchical distances given by $D$. 
%
%Specifically, $\Lproto$ is expressed as a cross-entropy between the hard-ranking ($ \bar{R}_{ijk}$) in the triplet of distances in $D$ and the soft-ranking $ R_{ijk}$ in the triplet of prototypes  (Eq. \ref{eq:lrank}). $ \bar{R}_{ijk}$ is given by Eq. \ref{eq:rbar} where $[\![ . ]\!]$ denotes the indicator function, and the soft-ranking $R_{ijk}$ is obtained by taking the sigmoid of the difference between the two distances in the embedding space. 
%
%\begin{align}
%    \Lproto(\pi) &= - \frac{1}{3 \cdot |\cT| } \sum_{(i,j,k) \in \cT} \left( \bar{R}_{ijk} \cdot \text{log}(R_{ijk}) + (1 - \bar{R}_{ijk}) \cdot \text{log}(1- R_{ijk}) \right) \label{eq:lrank} \\
%    & \cT \subset \{(i,j,k) \in \cK^3 | i \neq j, j \neq k , k\neq i \} \nonumber \\
%    \bar{R}_{ijk} & = [\![ D_{i,j} > D_{i,k} ]\!]  \label{eq:rbar}\\
%    R_{ijk} &= \text{sigmoid}(d(\pi_i,\pi_j) - d(\pi_i,\pi_k))  \label{eq:r}
%\end{align}
%
%
%For efficiency reasons we avoid computing this loss term over the complete set of triplets but randomly sample a fix-sized subset $\cT$ at each iteration. Lastly, the average cross-entropy is normalized by a factor $3$ in $\Lproto$ to balance its importance with $\Ldata$\footnote{For a perfectly balanced dataset, prototypes would otherwise occur three times more in the $\Lproto$ loss than in the $\Ldata$ term. }. 
%
}
{
% ALTERNATIVE 3.2 section

We propose to incorporate the cost matrix $D$ into a regularization term in order to encourage the prototypes
%We propose to incorporate the cost matrix $D$ into a regularization term.  \VIVIEN{It encourages} the prototypes  $\pi$ % \VIVIEN{, and indirectly the sample representations,} 
to organize in the embedding space $\Omega$ in a manner that is consistent with the finite metric defined by $D$. Since sample representations are attracted to their respective prototypes in \eqref{eq:ldata_long}, this regularization also affects the embedding network.
%
\paragraph{Scale-Free Distortion}
As described in \citet{de2018representation}, the distortion of a mapping $k \mapsto \pi_k$ 
between the finite metric space $(\cK, D)$ and  continuous metric space $(\Omega,d)$ can be defined as:
\begin{align}
\label{eq:disto}
\text{disto}(\pi,D) = \frac1{K(K-1)}
\sum_{k,l \in \cK^2,\,k\neq l} \frac{\left\vert d(\pi_{k},\pi_{l}) - D[k,l]\right\vert}{D[k,l]}~.
\end{align}
%Prototypes $\pi$ defining a low-distortion mapping are such that their pairwise distances $d$ are close to the misclassification costs defined by $D$.
\LOIC{A a sample $x_n$ of true class $k$ is incorrectly classified if $f(x_n)$ is closest to another prototype than to $\pi_k$. If the prototypes $\pi$ define a low-distortion mapping, then their pairwise distances $d$ are close to the misclassification costs defined by $D$. Consequently, misclassifying $x_n$ with a high-cost class $l_{\text{high}}$ would require $f(x_n)$ to be further away from $\pi_k$ than for another class with a lower cost $l_\text{low}$.}
%Consequently, misclassifying a sample $x_n$ of \LOIC{true} class $k$ with a high-cost class $l_{\text{high}}$ would require $f(x_n)$ to be further away from $\pi_k$ than for another class with a lower cost $l_\text{low}$.%\LOIC{ \ie $d(\pi_k, \pi_{l_\text{high}}) > d(\pi, \pi_{l_{\text{low}}})$}.
\LOIC{Hence, low-distortion prototypes arrangement are less prone to high-cost misclassifications, which could be advantageous in terms of AC.}
%Hence, by making high-cost misclassification less likely, a low-distortion arrangement could be advantageous in terms of AC.
%\LOIC{This leads us to regularize the classification model in order to favor low-distortion prototypes configurations.}
%This motivates us to regularize the classification model to favor low-distortion prototypes configurations.

%The same reasoning can apply to any homothetic mapping, yet the distortion defined in \equaref{eq:disto} only qualify 
However, achieving a low-distortion also imposes a specific scale on the distances between prototypes in the embedding space. 
This scale may conflict with the second term of $\Ldata$ which encourages distances between embeddings and unrelated prototypes to be as large as possible. \LOIC{Consequently, lower distortion may also cause lower precision. To remove this imposed scaling, we introduce a scale-independent formulation of the distortion:}
 \begin{align}
     \text{disto}^{\text{scale-free}}(\pi,D) = \min_{s \in \bR_+}{\text{disto}(s \cdot \pi, D)}~.
     \label{eq:scalefree}
 \end{align}
where $s \pi$ are the scaled prototypes, whose coordinates in $\Omega$ are multiplied by a scalar factor $s$.
% 
\paragraph{Distortion-Based Penalization}
%
%We propose to incorporate the error qualification in the prototypes' representations with a regularizer enforcing a low \emph{scale-free} distortion. \VIVIEN{Using a smooth surrogate we define the following regularizer: }
\LOIC{We propose to incorporate the error qualification $D$ into the prototypes' relative arrangement by encouraging a low \emph{scale-free} distortion between $\pi$ and $D$. To this end, we define the following smooth surrogate of \eqref{eq:scalefree} :}
%ooth surrogate
%enforcing a low \emph{scale-free} distortion. \VIVIEN{Using a smooth surrogate we define the following regularizer: }
\begin{align}
\label{eq:loss:distosmooth}
    \Ldisto(\pi) &= \frac{1}{K(K-1)} \min_{s \in \bR_+} %\left(
\sum_{k,l \in \cK^2,\,k\neq l} \left(\frac{ s \cdot d(\pi_{k},\pi_{l}) - D[k,l]}{D[k,l]}\right)^2 %\right)
~.
\end{align}
\LOIC{As described in the Appendix, $\Ldisto$ can be computed in closed form as a function of $\pi$ and can thus be directly used as regularizer.} 
%\VIVIEN{\equaref{eq:loss:disto} entails a simple case of bi-level optimization where the lower minimizer can be computed in closed form (see Appendix).} 
%\VIVIEN{
%RankNet \citep{ranknet}  inspired loss has also been proposed as a means of incorporating the class structure in the embedding space without imposing a fscale \citep{mettes2019hyperspherical}. We argue that the stronger supervision provided by out $\Ldisto$ is beneficial for the arrangement of the prototypes in the embedding space, see section \ref{sec:} for a comparison with a rank-based regularizer.}
%}
%
%
%\equaref{eq:scalefree} then implies a simple case of bi-level optimization where the lower minimizer can be computed in closed form:
%\begin{align}
%\label{eq:loss:minimizer}
%s^* &= \frac{\sum \frac{d(\pi_{k},\pi_{l})}{D[k,l]}}{\sum %\frac{d(\pi_{k},\pi_{l})^2}{D[k,l]^2}} ~.
%\end{align}

%This leads us to the following definition for our regularizer:
%\begin{align}
%\label{eq:loss:disto}
%    \Ldisto(\pi) &= \Lsurro(s^* \cdot \pi)
%\end{align}
%
%%
%\paragraph{Rank-based penalization} As proposed in RankNet \citep{ranknet}, encouraging the distances between prototypes to follow \emph{the same order} as the costs between their respective classes is another way to avoid a specific scaling:
%\begin{align}\label{eq:loss:rank}
%    \Lrank(\pi) &= - \frac{1}{\vert\cT\vert }
%\sum_{k,l,m \in \cT} %\left( 
%\bar{\bf R}_{k,l,m} \cdot \text{log}(R_{k,l,m}) + (1 - %\bar{\bf R}_{k,l,m}) \cdot \text{log}(1- R_{k,l,m}) %\right)
%~,
%\end{align}
%with $\cT=\{(k,l,m) \in  \cK^3\mid k\neq l, l\neq m, k\neq m\}$ the set of ordered triplet of $\cK$,  $\bar{\bf R}_{k,l,m}$ the hard ranking of the costs between $D_{k,l}$ and $D_{k,m}$, equal to $1$ if $D_{k,l} > D_{k,m} $ and $0$ otherwise, and $R_{k,l,m} = \text{sigmoid}(d(\pi_k,\pi_l) - d(\pi_k,\pi_m))$ the soft ranking between $d(\pi_k,\pi_l)$ and $d(\pi_k,\pi_m)$.
%For efficiency reasons, we sample at each iteration only a $S$-sized subset of $\cT$.
%%}
}
%..........................................
\subsection{End-to-end Training}
%..........................................
%We combine $\Ldata$ and a regularization $\Lmetric$ chosen as $\Ldisto$ or $\Lrank$ in a single loss $\La$ to jointly learn the embedding function $f$ and the class prototypes $\pi$:
We combine $\Ldata$ and  $\Ldisto$ in a single loss $\La$ to jointly learn the embedding function $f$ and the class prototypes $\pi$:
\begin{equation}
    \La(f, \pi) = \Ldata(f, \pi) + \lambda \cdot \Ldisto(\pi)~, \label{eq:loss:total}
\end{equation}
with $\lambda\in \bR_+$ an hyper-parameter setting the strength of the regularization.
%................................................
\subsection{Choosing a Metric Space}
%................................................
Prototypical networks operating on $\Omega=\bR^d$ typically use the squared Euclidean norm in the distance function, motivated by its quality as a Bregman divergence  \citep{snell2017prototypical}.
%However, given that the metric penalizers tends to produce prototypes which are further apart than their unguided counterparts, the square norm made learning less stable learni
However, we observe that defining $d$ with the Euclidean norm yields significantly better results. The non-differentiability can be handled by composing with a Huber-like \citep{huber1973robust, charbonnier1997deterministic} function $d={H}(\lVert \cdot \rVert)$, with $H$ defined as:
\begin{equation}
    {H}(x) = \delta (\sqrt{\Vert x \Vert^2 / \delta^2+1}-1)~, \label{eq:ph}
\end{equation}
and $\delta\in\bR_+$ a (small) hyper-parameter. The resulting metric $d$ is asymptotically equivalent to the Euclidean norm for large distances, and behaves like the smooth squared Euclidean norm for small distances. In \secref{sec:ablation}, we investigate  the effect of this change, as well as its parameterization.
%
%
%\VIVIEN{As shown in \eqref{eq:ph}, such a function is asymptotically equivalent to the euclidean norm, and behaves like the squared norm close to zero. In light of the little effect this had on our results (see \ref{sec:ablation}) we kept the Euclidean norm throughout the numerical experiments.} 
\ANY{}{
%................................................
\subsection{Inference}
%................................................
\label{sec:inference}
As with other prototypical networks, we associate to a sample $n$ the class $k$ whose prototype $\pi_k$ is the closest to the representation $f(x_n)$ with respect to $d$, corresponding to the class of highest probability.
This process can be made efficient for a large number of classes $K$ and a high embedding dimension $m$ with a KD-tree data structure, which offers a query complexity of $O(\log(K))$ instead of $O(K\cdot m)$ for an exhaustive comparison. Hence, our method does not induce longer inference time than the cross-entropy for example, as the embedding function typically takes up the most time.
}
%
 \ANY{}{\paragraph{Any-Node Inference:} %
Choosing the class of highest probability maximizes the accuracy of the prediction.
%
However, when the average cost is the focus, this may not be the best strategy.
%
Indeed, as suggested by \citet{deng2010does}, one can instead chose the class $k$ which minimize the \emph{Expected Cost} $\text{EC}(k\mid x)$ given an observation $x_n \in \cX$:
\begin{align}\label{eq:expcost}
    \text{EC}(k\mid x_n) 
    &
    =
    \mathbb{E}_{l\sim p(y_n=k\mid x_n)}D[k,l]
    =
    \sum_{l \in \cK} p(y_n = l \mid x_n) \cdot D[k,l]~.% \label{eq:expcost}\\
    %\Tilde{y} &= \text{argmin}_{k \in \cK} \{ \text{ExC}[k ] \}
\end{align}
Across our experiments, this scheme showed little difference compared to choosing the class with highest probability.%, as shown in \ref{sec:ablation}.
}

 \ANY{}{When the cost matrix $D$ is derived from a tree-shaped hierarchy of class, we can distinguish between \emph{leaf-classes} corresponding to leaf nodes, and \emph{internal-classes}.
In most classification tasks, all sample are labeled as leaf-classes, and hence predicting an internal-class is always detrimental to the accuracy.
However, when leaf-class confidences are low (\eg hesitating between $10$ dog breeds), it can be beneficial in terms of AC to predict the parent class (\eg simply choosing the \emph{dog} class).
}

\ANY{}{We denote by $\bar{\cK}$ the set containing both internal and leaf-classes. We define the any-node prediction scheme as:
\begin{equation}
    \bar{z} = \text{argmin}_{k \in \bar{\cK}} \text{EC}(k\mid x_n)~. \label{eq:anynode}
\end{equation}
In our experiments, network calibration \citep{guo2017calibration} had little impact on the quality of results, and was hence omitted for the sake of simplicity.
}
%
%\paragraph{Probability based inference} The predicted class at inference time is that with the highest predicted probability \ie  the class of the closest prototype to the sample embedding \eqref{eq:maxP}.
%
%\begin{equation}
%    \hat{y} = \text{argmin}_{k \in \cK} \{d(f(x), \pi_k)\} \label{eq:maxP}
%\end{equation}
% While we have not implemented it, we note that inference could be optimized for large nomenclatures by finding the closest prototype using a KD-tree algorithm.   
%
%\paragraph{Minimum hierarchical cost inference} Furthermore, we propose an alternative inference method for settings where minimizing the AHC of predictions is more important than overall accuracy. The pseudo-probabilities defined in \eqref{eq:proba} can be used to implement an \textit{expected cost minimizing} inference scheme. Assuming that the class labels follow the distribution defined by the pseudo-probabilities, the expected hierarchical cost of predicting class $k$ is given by:
%\begin{align}
%    \text{ExC}[ k ] &= \sum_{l \in \cK} p(y = l | x) \cdot D_{k,l} \label{eq:expcost}\\
%    \Tilde{y} &= \text{argmin}_{k \in \cK} \{ \text{ExC}[k ] \}
%\end{align}
%
%
%This framework of inference can easily be extend to non-mandatory leaf node (NML) prediction. The expected cost (Eq. \ref{eq:expcost}) can indeed be computed for any class $k \in \bar{\cK}$ in the extended set of class labels containing the internal nodes of the tree.
%\begin{equation}
%    \Tilde{y}_{NML} = \text{argmin}_{k \in \bar{\cK}} \{ \text{ExC}[k ] \}
%\end{equation}
%
%Using the cost matrix $D$ to implement such a NML inference scheme is a simple way to reduce the AHC even further at the cost of having higher-level prediction when leaf-level class confidences are not high enough to make up for the potential cost of misclassification. 

==> bri.tex <==
\section*{Broader Impact}
The impact of this work concerns mainly applications for which some error types can have serious consequences, such as autonomous navigation and fraud detection.

As for broader societal consequences, incorporating an external error qualification directly into the learning process can have both a positive and negative effect depending on its use. If the cost matrix integrates misconceptions or prejudiced information, they will be reflected in the algorithm's inner working. On the other hand, if $D$ is specifically chosen to insure fairness, it may be a way to discourage the implicit use of problematic latent variables.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}



% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

